NorBERT: NetwOrk Representations through BERT for Network Analysis and Management

Deep neural network models have been very successfully applied to Natural Language Processing (NLP) and Image based tasks. Their application to network analysis and management tasks is just recently being pursued. Our interest is in producing deep models that can be effectively generalized to perform well on multiple network tasks in different environments. A major challenge is that traditional deep models often rely on categorical features, but cannot handle unseen categorical values. One method for dealing with such problems is to learn contextual embeddings for categorical variables used by deep networks to improve their performance. In this paper, we adapt the NLP pre-training technique and associated deep model BERT to learn semantically meaningful numerical representations (embeddings) for Fully Qualified Domain Names (FQDNs) used in communication networks. We show through a series of experiments that such an approach can be used to generate models that maintain their effectiveness when applied to environments other than the one in which they were trained.

==> related.tex <==
\section{Related Work}

To the best of the authors' knowledge, this paper is the first to explore the creation of contextual embeddings for network categorical variables, and to evaluate them. 

In~\cite{Antoine2020NetBERTAP}, Antoine introduces NetBERT, a domain-specific language representation model based on BERT, and pre-trained using a large-scale computer networking corpora. In other words, that paper proposes a model that learns embeddings for computer networking lexicon. That model is still related to neural language processing. In contrast, NorBert learns contextual embeddings for network categorical variables in actual IP packets.

The closest work to NorBert is ~\cite{Le2019UnearthingAE}, where Le and Srivatsa proposed an algorithm to calculate context independent embeddings for FQDNs. However, the results of Section~\ref{sec:results} show that contextual embeddings significantly outperform context independent embeddings for downstream tasks (e.g., device classification).
